Sensing-Aided Near-Field Beam Tracking

The interplay between large antenna apertures and high carrier frequencies in future wireless systems gives rise to near-field communications, where the curvature of spherical wavefronts renders traditional far-field beamforming models inadequate. This chapter addresses the following fundamental questions on near-field operation: (i) What is the maximum distance where far-field approximations remain effective for path gain prediction and beam design? (ii) What level of position resolution is needed for accurate near-field beam focusing? (iii) How frequently must channel state information be updated to maintain highly directive bweamforming in dynamic scenarios? We develop an analytical framework for assessing near-field beamforming gain degradation due to mismatches between the focusing point and the coordinates of a user. Closed-form expressions for beam correlation, beam sensitivity to user movement, and the direction of fastest beamforming gain degradation are derived. A dynamic polar coordinate grid is also proposed for low complexity and adaptive near-field beam search. Furthermore, we introduce the novel concept of beam coherence time, quantifying the temporal robustness of focused beams and enabling proactive sensing-aided beam tracking strategies. The effect of microstrip losses on the preceding derivations is also analyzed. Finally, extensive simulation results validate the presented theoretical analysis and beam tracking method over randomly generated user trajectories.

==> editor/acknowledgement.tex <==
%%%%%%%%%%%%%%%%%%%%%%acknow.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample acknowledgement chapter
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acknowledgements}

Use the template \emph{acknow.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) if you prefer to set your acknowledgement section as a separate chapter instead of including it as last part of your preface.



==> editor/acronym.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer Nature%%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acronyms}

Use the template \emph{acronym.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your list(s) of abbreviations or symbols.

Lists of abbreviations\index{acronyms, list of}, symbols\index{symbols, list of} and the like are easily formatted with the help of the Springer Nature enhanced \verb|description| environment.

\begin{description}[CABR]
\item[ABC]{Spelled-out abbreviation and definition}
\item[BABI]{Spelled-out abbreviation and definition}
\item[CABR]{Spelled-out abbreviation and definition}
\end{description}
